BigGait: Learning Gait Representation You Want by Large Vision Models

Gait recognition stands as one of the most pivotal remote identification technologies and progressively expands across research and industry communities. However, existing gait recognition methods heavily rely on task-specific upstream driven by supervised learning to provide explicit gait representations like silhouette sequences, which inevitably introduce expensive annotation costs and potential error accumulation. Escaping from this trend, this work explores effective gait representations based on the all-purpose knowledge produced by task-agnostic Large Vision Models (LVMs) and proposes a simple yet efficient gait framework, termed BigGait. Specifically, the Gait Representation Extractor (GRE) within BigGait draws upon design principles from established gait representations, effectively transforming all-purpose knowledge into implicit gait representations without requiring third-party supervision signals. Experiments on CCPG, CAISA-B* and SUSTech1K indicate that BigGait significantly outperforms the previous methods in both within-domain and cross-domain tasks in most cases, and provides a more practical paradigm for learning the next-generation gait representation. Finally, we delve into prospective challenges and promising directions in LVMs-based gait recognition, aiming to inspire future work in this emerging topic. The source code is available at https://github.com/ShiqiYu/OpenGait.

==> supply/7_supply.tex <==

\begin{table*}[h!]
\centering
\caption{Ablation of denoising branch: exploring channel number, and w/ and w/o smoothness and diversity loss.}
\renewcommand{\arraystretch}{1}
% \Huge
\resizebox{1.6\columnwidth}{!}{

\begin{tabular}{c|cccc|ccc|ccc} 
\toprule[2pt]
\multirow{3}{*}{Model} & \multicolumn{10}{c}{Self-domian Evaluation}                                                                                                                     \\ 
\cline{2-11}
                       & \multicolumn{4}{c|}{CCPG}                                     & \multicolumn{3}{c|}{CASIA-B*}                  & \multicolumn{3}{c}{SUSTech1K}                  \\ 
\cline{2-11}
                       & CL            & UP            & DN            & BG            & NM             & BG            & CL            & Clothing      & Night         & Overall        \\ 
% \hline
\midrule[1pt]
GaitBase               & 60.2          & 65.2          & 65.1          & 68.5          & 92.3           & 86.1          & 73.4          & 39.4          & 24.0          & 67.1           \\
GaitEdge               & 71.6          & 75.0          & 76.8          & 78.6          & 96.5           & 91.5          & 78.0          & 47.2          & 26.4          & 75.8           \\
AP3D                   & 53.4          & 57.3          & 69.7          & 91.4          & 99.8           & \textbf{99.4} & \textbf{87.6} & \textbf{82.7} & \textbf{89.4} & \textbf{96.8}  \\
PSTA                   & 42.2          & 52.2          & 60.3          & 84.5          & 98.2           & 96.5          & 54.2          & 72.3          & 79.9          & 93.6           \\
BigGait                & \textbf{76.0} & \textbf{79.1} & \textbf{84.2} & \textbf{93.0} & \textbf{100.0} & \textbf{99.4} & 86.4          & 69.8          & 84.1          & 96.2           \\
\bottomrule[2pt]
\end{tabular}

}
\label{tab: Denoising Branch}
\end{table*}


\section{Supplementary Material}
\label{sec: Supplementary Material}
% In this section,
% we first explore the effectiveness of several usual spatial
% data augmentation operations. Then, we conduct comprehensive experiments to analyze the effect of random training input length. Lastly, we talk about some future works
% that are worth further exploration.

In this section, we first provide the self-domain results on CASIA-B* and SUSTech1K.
Then, we conduct more visualization to analyze the difference between
BigGait and video-based ReID methods.





\subsection{More Self-domain Results}



